Validating Streaming JSON Documents with Learned VPAs

We present a new streaming algorithm to validate JSON documents against a set of constraints given as a JSON schema. Among the possible values a JSON document can hold, objects are unordered collections of key-value pairs while arrays are ordered collections of values. We prove that there always exists a visibly pushdown automaton (VPA) that accepts the same set of JSON documents as a JSON schema. Leveraging this result, our approach relies on learning a VPA for the provided schema. As the learned VPA assumes a fixed order on the key-value pairs of the objects, we abstract its transitions in a special kind of graph, and propose an efficient streaming algorithm using the VPA and its graph to decide whether a JSON document is valid for the schema. We evaluate the implementation of our algorithm on a number of random JSON documents, and compare it to the classical validation algorithm.

==> figures/VPA/accepted_tree.tex <==
\begin{tikzpicture}[
    tree,
    level 1/.style = {sibling distance = 20mm},
    level 2/.style = {sibling distance = 10mm}
]
    \node [
        state,
        label={[runColor]left:\(q\)},
        label={[runColor]right:\(q'\)}
    ] (root) {\(a\)}
        child {
            node [
                state,
                label={[runColor]left:\(s_1\)},
                label={[runColor]right:\(s_2\)}
            ] (b1) {\(b_1\)}
            child [dashed,-] {
                node {\(\vdots\)}
            }
            child [dashed,-] {
                node {\(\vdots\)}
            }
        }
        child {
            node [
                state,
                label={[runColor]right:\(s_3\)}
            ] (b2) {\(b_2\)}
            child [dashed,-] {
                node {\(\vdots\)}
            }
            child [dashed,-] {
                node {\(\vdots\)}
            }
        }
        child {
            node [
                state,
                label={[runColor]right:\(s_4\)}
            ] (b3) {\(b_3\)}
            child [dashed,-] {
                node {\(\vdots\)}
            }
            child [dashed,-] {
                node {\(\vdots\)}
            }
        }
    ;

\end{tikzpicture}

==> futureWork.tex <==
\section{Future work}\label{sec:future}
